Predicting Object Interactions with Behavior Primitives: An Application in Stowing Tasks

Stowing, the task of placing objects in cluttered shelves or bins, is a common task in warehouse and manufacturing operations. However, this task is still predominantly carried out by human workers as stowing is challenging to automate due to the complex multi-object interactions and long-horizon nature of the task. Previous works typically involve extensive data collection and costly human labeling of semantic priors across diverse object categories. This paper presents a method to learn a generalizable robot stowing policy from predictive model of object interactions and a single demonstration with behavior primitives. We propose a novel framework that utilizes Graph Neural Networks to predict object interactions within the parameter space of behavioral primitives. We further employ primitive-augmented trajectory optimization to search the parameters of a predefined library of heterogeneous behavioral primitives to instantiate the control action. Our framework enables robots to proficiently execute long-horizon stowing tasks with a few keyframes (3-4) from a single demonstration. Despite being solely trained in a simulation, our framework demonstrates remarkable generalization capabilities. It efficiently adapts to a broad spectrum of real-world conditions, including various shelf widths, fluctuating quantities of objects, and objects with diverse attributes such as sizes and shapes.

==> Sections/02-RelatedWorks.tex <==
\section{Related Works}
\subsection{One-shot imitation learning } 
% - Kaiwen, Shuijing
% (previous methods work bad cause  no models. what's the limitation in no models in imitation learning )

% possibly mention dagger ?:https://ieeexplore.ieee.org/abstract/document/8793698

% https://arxiv.org/pdf/2111.07447.pdf
% https://proceedings.mlr.press/v87/james18a.html
% https://arxiv.org/abs/2201.12716
% https://proceedings.neurips.cc/paper/2017/hash/ba3866600c3540f67c1e9575e213be0a-Abstract.html
% https://proceedings.mlr.press/v164/jang22a.html
% https://proceedings.mlr.press/v78/finn17a.html

Recent one-shot imitation learning methods aim to solve a task with only one demonstration. \cite{NIPS2017_ba386660} adopt a two-phase pipeline, with a meta-learning phase training a general policy based on a large number of tasks and then a fine-tuning phase, which optimizes the policy for the specific task at hand using the single provided demonstration. \cite{valassakis2022demonstrate} proposes a simple yet effective replay-based method but it cannot exceed the demonstration performance. Others find correspondence of particular objects \cite{chai2019multi}, \cite{ganapathi2021learning} or objects in the same category \cite{wen2022you} for manipulation but the task is relatively short-horizon.

\subsection{Model learning in robo mani}% - Yixuan
% (given the previous imitation learning why do we want to learn model, how to do model choices)

Dynamics models have recently become one key component of robotic systems. Typically, a dynamics model takes in current world states and actions and predicts the world states in the future. The dynamics model could take in representations with various forms, including images~\cite{suh2021surprising}, latent vectors~\cite{yan2021learning}, point set~\cite{manuelli2020keypoints,mitrano2021learning}, and graphs~\cite{shi2022robocraft,lin2022learning,huang2022mesh}. The graph has demonstrated the ability to capture the interaction between multiple objects~\cite{li2018learning,li2019propagation,battaglia2016interaction,chang2016compositional,sanchez2018graph,funk2022learn2assemble,silver2021planning}. In our case, we would like to model the interaction between multiple objects and the robot end effector. Therefore, we choose to use the graph to model the interaction in our system.

\subsection{Long-horizon planning in robo mani}
% - Kaiwen
 % (we have seen model learning in robo mani, why just one model is not enough )
Solving long-horizon manipulation problems is challenging. Hierarchical reinforcement learning tackles the problem with a higher-level policy of choosing the optimal subtasks and low-level policies are then trained to execute them \cite{gupta2019relay}. However, data collection and the sim2real gap make the policy hard to transfer to the real world. \cite{di2022learning} uses a replay-based approach to solve everyday long-horizon tasks but the task configuration lacks variants. Recently, \cite{lin2022diffskill} tackles the sequential manipulation of deformable objects with differential simulator and trajectory optimization but this work is only validated in the simulator and deploying it to the real-world is also challenging and non-trivial.
 


==> Sections/06-Limitations <==
\section{Limitations}
\label{sec:limitations}

Our system currently has a few limitations. Firstly, it relies on manual human labeling of ordered keyframes from demonstrations, which could potentially restrict scalability and deployment in larger and more complex scenarios. Secondly, we use box-shaped point clouds to represent objects during training and inference. This simplistic representation may not accurately reflect the geometrical properties of objects, especially in scenarios involving more complex interactions and contacts. Addressing these limitations, particularly improving object representation, presents a promising direction for future research.



% box shaped objects
% Additionally, the system currently lacks the capability to autonomously select the most appropriate skill. Instead, it relies on skill information extracted directly from human demonstrations, which restricts the system's ability to retroactively evaluate errors from prior timestamps and correct them in real-time.


==> figText/setup.tex <==

\begin{figure}[htb]
    \begin{minipage}{0.6\textwidth}
        \centering
        \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\textwidth]{Figures/000_setup_low.png}
            \caption{}
        \end{subfigure}%
        ~
        \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\textwidth]{Figures/001_setup_low.png}
            \caption{}
        \end{subfigure}
        ~ 
        \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\textwidth]{Figures/002_setup_low.png}
            \caption{}
        \end{subfigure}
        
        \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\textwidth]{Figures/003_setup_low.png}
            \caption{}
        \end{subfigure}%
        ~ 
        \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\textwidth]{Figures/004_setup_low.png}
            \caption{}
        \end{subfigure}
        ~ 
        \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\textwidth]{Figures/005_setup_low.png}
            \caption{}
        \end{subfigure}
        % \label{fig:setup}
    \end{minipage}
    % \hspace{0.1cm}
    \begin{minipage}{0.4\textwidth}
        \centering
        % \resizebox{\textwidth}{!}{ % This will resize the table to fit the width of the minipage
            \begin{tabular}{cccc}
            \toprule
            \multirow{2}{0.8cm}{Setups} & \multicolumn{3}{c}{Success ($\uparrow$)} \\
             & Heuristic & 3 skills & 2 skills \\
            \cmidrule(lr){1-1} \cmidrule(lr){2-4}
            (a) & 1/10 & 10/10 & 10/10\\
            (b) & 2/10 & 10/10 & 10/10 \\
            (c) & 1/10 & 10/10 & 10/10\\
            (d) & 3/10 & 9/10 & 9/10\\
            (e) & 3/10 & 9/10 & 9/10\\
            (f) & 1/10 & 9/10 & 9/10\\
            \cmidrule(lr){1-1} \cmidrule(lr){2-4}
            Average & 18\% & 95\% & 95\%\\
            \bottomrule
            \end{tabular}
        % }
            % \captionof{table}{}
    \label{tab:control_quantitative}
    \end{minipage}
        \caption{\textbf{Left: }Different Setups Used in Real-World Manipulation Experiments. Six setups represent a wide range of conditions including different combinations of objects, shelf sizes, object dimensions, and shapes. (a) A setup with three boxes in the shelf and one box on the table. (b) A setup featuring one roller in the shelf and one bottle on the table. The non-box shape and plastic material of the roller and bottle increase the challenge due to their slippery nature. (c) A setup with four boxes in the shelf, designed to test our method's ability to handle multiple object interactions. (d) A setup featuring a small sugar box, examining our method's ability to manage objects with significant size differences. (e) A setup featuring a thin but heavy book and a trapezoid box, which introduces more complex dynamics. (f) A setup with a narrow shelf width, aimed at testing the generalization ability of our framework with varying shelf width. \textbf{Right: }Success Rates of Control Actions in Real-World Environments. The performance of our proposed method, using two different skill sets (2-skill and 3-skill) and a heuristic-based control action selection, is evaluated across six different setups. }
        \label{fig:setup_success}
    \vspace{-10pt}
\end{figure}
